The Maximal MAM, a Reasonable Implementation of the Maximal Strategy

This note is about a reasonable abstract machine, called Maximal MAM, implementing the maximal strategy of the lambda-calculus, that is, the strategy that always produces a longest evaluation sequence.

==> proofs/commutative-distallation-proof-old.tex <==
% !TEX root = ../main.tex
%\myproof{
\begin{proof}
\hfill
\begin{itemize}
\item \case{$\mac{ \skeval }{ \skframe }{ \code\codetwo }{ \stack }{ \genv }
             \tomachasubone
             \mac{ \skeval }{ \skframe }{ \code }{ \codetwo\cons\stack }{ \genv }$}
     \[\begin{array}{lllllllll}
     
     \decode{\mac{ \skeval }{ \skframe }{ \code\codetwo }{ \stack }{ \genv } }
     &=&
     \decdump\ctxholep{\decstackp{\code\codetwo}}\indsub\genv
     &=&
          \decdump\ctxholep{\decodep{\codetwo\cons\stack}{(\code\codetwo)}}\indsub\genv
          &=&
     
     \decode{ \mac{ \skeval }{ \skframe }{ \code }{ \codetwo\cons\stack }{ \genv } }
 \end{array}\]


\item \case{$\mac{ \skeval }{ \skframe}{ \la\var\code }{ \stempty }{ \genv }
             \tomachasubtwo
             \mac{ \skeval }{ \mframe\cons\var }{ \code }{ \stempty }{ \genv }$}
    \[\begin{array}{lllllllll}
    &
    \decode{\mac{ \skeval }{ \skframe}{ \la\var\code }{ \stempty }{ \genv }}
    &=&
     \decodep{\mframe}{\la\var\code}\indsub\genv
    &=&
     \decodep{\mframe\cons\var}\code\indsub\genv
    &=&
    \decode{\mac{ \skeval }{ \mframe\cons\var }{ \code }{ \stempty }{ \genv }}
    \end{array}\]

\item \case{$\mac{ \skeval }{ \skframe }{ \var }{ \stack }{ \genv }
             \tomachasubthree
             \mac{ \skback }{ \skframe }{ \var }{ \stack }{ \genv }$}
The decoding does not depend on the phase, so 
     $\decode{\mac{ \skeval }{ \skframe }{ \var }{ \stack }{ \genv }}
     =
     \decode{\mac{ \skback }{ \skframe }{ \var }{ \stack }{ \genv }}$.

\item \case{$\mac{ \skback }{ \mframe\cons\var }{ \code }{ \stempty }{ \genv }
             \tomachasubfour
             \mac{ \skback }{ \skframe }{ \la\var\code }{ \stempty }{ \genv }
             $}
             Since the decoding does not depend on the phase, this case goes exactly as $\tomachasubtwo$:
    \[\begin{array}{lllllllll}
    &
    \mac{ \skback }{ \mframe\cons\var }{ \code }{ \stempty }{ \genv }
    &=&
     \decodep{\mframe\cons\var}\code\indsub\genv
    &=&
     \decdumpp{\la\var\code}\indsub\genv
    &=&
    \mac{ \skback }{ \skframe }{ \la\var\code }{ \stempty }{ \genv }
    \end{array}\]

\item \case{$			\mac{ \skback }{ \skframe\cons \dentry\code\stack  }{ \codetwo }{ \stempty }{ \genv }
             \tomachasubfive
             \mac{ \skback }{ \skframe }{ \code\codetwo }{ \stack }{ \genv }$}
        \[\begin{array}{lllllllll}
     
     \decode{\mac{ \skback }{ \skframe\cons \dentry\code\stack  }{ \codetwo }{ \stempty }{ \genv }}
     &=&
               \decodep{ (\skframe \cons \dentry\code\stack)}\codetwo \indsub\genv
     &=&\\
     &=&               \decdump\ctxholep{\decstackp{\code\codetwo}}\indsub\genv
          &=&\\
     &=&
\decdump\ctxholep{\decodep{\codetwo\cons\stack}{\code}}\indsub\genv
     &=&
     \decode{\mac{ \skback }{ \skframe }{ \code\codetwo }{ \stack }{ \genv }}
     \end{array}\]
     
\item \case{$\mac{ \skback }{ \skframe }{ \code }{ \codetwo\cons\stack }{ \genv }
             \tomachasubsix
             \mac{ \skeval }{ \skframe \cons \dentry\code\stack }{ \codetwo }{ \stempty }{ \genv }$}
                          Since the decoding does not depend on the phase, this case goes exactly as $\tomachasubfive$:
    \[\begin{array}{lllllllll}
     
     \decode{\mac{ \skback }{ \skframe }{ \code }{ \codetwo\cons\stack }{ \genv }}
     &=&
          \decdump\ctxholep{\decodep{\codetwo\cons\stack}{\code}}\indsub\genv
     &=&\\
     &=&               \decdump\ctxholep{\decstackp{\code\codetwo}}\indsub\genv
          &=&\\
     &=&
     \decodep{ (\skframe \cons \dentry\code\stack)}\codetwo \indsub\genv
     &=&
     \decode{\mac{ \skeval }{ \skframe \cons \dentry\code\stack }{ \codetwo }{ \stempty }{ \genv }}
     \end{array}\]\qed
\end{itemize}
\end{proof}
%}

==> proofs/invariant-proof-schema.tex <==
% !TEX root = ../main.tex
\begin{proof}
  The invariant trivially holds for an initial state
  $\skamstate{\skeval}{\stempty}{\code}{\stempty}{ \stempty}$.
For a non-empty evaluation sequence we list the cases for the last transition. 

\begin{itemize}

  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \item Principal Cases:

   \begin{itemize}
    \item \case{$\statetwo = 
          \mac{ \skeval }{ \skframe }{ \l\var.\code }{ \vartwo\cons\stack }{ \genv }
          \tomachmone
          \mac{ \skeval }{ \skframe }{ \code\isub\var\vartwo }{ \stack }{ \genv } = \state
        $}

			
    \item \case{$\statetwo = 
          \mac{ \skeval }{ \skframe }{ \l\var.\code }{ \codetwo\cons\stack }{ \genv }
          \tomachmtwo
          \mac{ \skeval }{ \skframe }{ \code }{ \stack }{ \esublab{\var}{\codetwo}\cons\genv } = \state
        $ with $\codetwo$ not a variable}
			

			
    \item \case{$\statetwo = 
          \mac{ \skeval }{ \skframe }{ \var }{ \stack }{ \genv }
          \tomachered
          \mac{ \skeval }{ \skframe }{ \rename{\code} }{ \stack }{ \genv } = \state$ with $\genv(\var) = \esublabe\var\codetwo{\labred n}$}
        
    \item \case{$\statetwo = 
          \mac{ \skeval }{ \skframe }{ \var }{ \codetwo\cons\stack }{ \genv }
          \tomacheabs
          \mac{ \skeval }{ \skframe }{ \rename{\code} }{ \codetwo\cons\stack }{ \genv } = \state$ with $\genv(\var) = \esublabe\var\codetwo\lababs$}
  \end{itemize}
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

 \item Commutative Cases:
  \begin{itemize}
 \item \case{$\statetwo = 
          \mac{ \skeval }{ \skframe }{ \code\codetwo }{ \stack }{ \genv }
          \tomachasubone
          \mac{ \skeval }{ \skframe }{ \code }{ \codetwo\cons\stack }{ \genv } = \state
        $}
 
%    \begin{enumerate}
%	\item
%    \end{enumerate}
  
  \item \case{$\statetwo = 
          \mac{\skeval}{\skframe}{\la\var\code}{\stempty}{\genv}
          \tomachasubtwo
          \mac{\skeval}{\skframe\cons\var}{\code}{\stempty}{\genv} = \state
        $}
        
%    \begin{enumerate}
%	\item
%    \end{enumerate}

  \item \case{$\statetwo = 
          \mac{\skeval}{\skframe}{\var}{\stack}{\genv}
          \tomachasubthree
          \mac{\skback}{\skframe}{\var}{\stack}{\genv} = \state
        $ with $\genv(\var) = \bot$ or $\genv(\var) = \esublabe\var\codetwo\labneu$ or ($\genv(\var) = \esublabe\var\codetwo\lababs$ and $\stack = \stempty$)
        }
    
    Three cases depending on $\genv$:
      \begin{enumerate}
	\item $\genv(\var) = \bot$: 
	\item $\genv(\var) = \esublabe\var\codetwo\labneu$: 
	\item $\genv(\var) = \esublabe\var\codetwo\lababs$ and $\stack = \stempty$: 
      \end{enumerate}
      
%    \begin{enumerate}
%	\item
%    \end{enumerate}

  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \item \case{$\statetwo = 
          \mac{\skback}{\skframe\cons\var}{\code}{\stempty}{\genv}
          \tomachasubfour
          \mac{\skback}{\skframe}{\la\var\code}{\stempty}{\genv} = \state
        $}
    
    
%    \begin{enumerate}
%	\item
%    \end{enumerate}

  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \item \case{$\statetwo = 
          \mac{\skback}{ \skframe\cons\skap{\code}{\stack} }{\codetwo}{\stempty}{\genv}
          \tomachasubfive
          \mac{\skback}{\skframe}{\code\codetwo}{\stack}{\genv} = \state
        $}

%    \begin{enumerate}
%	\item
%    \end{enumerate}

  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \item \case{$\statetwo = 
          \mac{\skback}{\skframe}{\code}{\codetwo\cons\stack}{\genv}
          \tomachasubsix
          \mac{\skeval}{ \skframe\cons\skap{\code}{\stack} }{\codetwo}{\stempty} {\genv} = \state
        $}
%    \begin{enumerate}
%	\item
%    \end{enumerate}
        
   \end{itemize}
  \end{itemize}
\end{proof}
